You Only Need One Step: Fast Super-Resolution with Stable Diffusion via Scale Distillation

In this paper, we introduce YONOS-SR, a novel stable diffusion-based approach for image super-resolution that yields state-of-the-art results using only a single DDIM step. We propose a novel scale distillation approach to train our SR model. Instead of directly training our SR model on the scale factor of interest, we start by training a teacher model on a smaller magnification scale, thereby making the SR problem simpler for the teacher. We then train a student model for a higher magnification scale, using the predictions of the teacher as a target during the training. This process is repeated iteratively until we reach the target scale factor of the final model. The rationale behind our scale distillation is that the teacher aids the student diffusion model training by i) providing a target adapted to the current noise level rather than using the same target coming from ground truth data for all noise levels and ii) providing an accurate target as the teacher has a simpler task to solve. We empirically show that the distilled model significantly outperforms the model trained for high scales directly, specifically with few steps during inference. Having a strong diffusion model that requires only one step allows us to freeze the U-Net and fine-tune the decoder on top of it. We show that the combination of spatially distilled U-Net and fine-tuned decoder outperforms state-of-the-art methods requiring 200 steps with only one single step.

==> sec/4x_arch_distillation.tex <==
\subsection{Scale distillation for architecture distillation}\label{sec:arch-distill}
We have shown so far that YONOS-SR is able to generate high-quality images with a single inference step. However, the UNet used in stable diffusion framework v1.5 is a relatively big model, containing $860$M parameters. Using such a big model on low-budget computing devices such as cell phones, even for a single step for each image patch, is still expensive. In this section, we show how we can adapt the proposed scale distillation approach to training a smaller stable diffusion-based super-resolution (SD-SR) model, resulting in not only a fast model in terms of the number of steps but also a parameter and resource-efficient model. 
%Specifically, our goals here are twofold. We aim to show that \textbf{i)} the proposed scale distillation approach also generalizes to smaller model sizes. \textbf{ii)} the same strategy of simplifying the problem in a training diffusion model for super resolution through scale distillation, can be adapted to train smaller model through architecture distillation.


\begin{table}[t]
\resizebox{0.99\linewidth}{!}{
    \centering
    \begin{tabular}{cc|cccc}
         \toprule
         \makecell{Architecture \\ distillation} & \makecell{Scale \\ distillation} & FID $\downarrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ \\
         \hline
         \xmark & \xmark & 43.39 & 0.3266 & 25.38 & 0.6934 \\
        \xmark & \checkmark & 32.24  & 0.2634 & 26.23 & 0.7076 \\
         \checkmark & \xmark & 34.76 & 0.2683 & 25.46 & 0.6972  \\
        \checkmark & \checkmark & \textbf{28.57} & \textbf{0.2518} & \textbf{26.55} &  \textbf{0.7155} \\
        \hline
         \multicolumn{2}{c|}{Big model with scale distillation}& 21.63& 0.2100& 25.06 & 0.691\\
        \bottomrule
    \end{tabular}
}
    \caption{Role of the proposed scale and architecture distillation in training a small model. No decoder fine-tuning is performed here. All results are obtained with one inference step using the $3000$ random crops of DIV2K  bicubic degradation for $\times 4$ magnification.
    The small model trained directly for $\times 4$ magnification without any distillation-based training(first row) suffers a significant performance drop compared to the big model with scale distillation. Introducing either scale (second row) or architecture(third row) distillation significantly improves the results. A combination of both with architecture distillation on a lower scale factor and scale distillation from that improves the performance further(fourth row).}
    \label{tab:arch-distill}
\end{table}

\begin{algorithm}[ht]
\begin{algorithmic}[1]
\State Input: dataset $\mathcal{D}$ 
\State Input: noise schedule $\alpha_t, \sigma_t, \lambda_t$ \Comment{for $t \in [0,1]$}
\State Input: scale factor $s$ 
\State Input: initialization $\theta$ \Comment{small student weights}
\State Input: initialization $\phi$ \Comment{big pre-trianed teacher}

\While{not converged} \Comment{student training}
    \State $t \sim \mathcal{U}[0,1]$
    \State $\epsilon \sim \mathcal{N}(0,I)$
    \State $\mathbf{x}_h \sim \mathcal{D}$ 
    \State $\mathbf{x}_l \gets \Call{Degrade}{\mathbf{x}_h,s}$ 
    \State $\mathbf{z}_h \gets \mathcal{E}(\mathbf{x}_h)$
    \State $\mathbf{z}_l \gets \mathcal{E}(\Call{ResizeLike}{\mathbf{x}_l,\mathbf{x}_h})$
    \State $\mathbf{z}_t \gets \alpha_t \mathbf{z}_h + \sigma_t \epsilon$
    \State $\tilde{\mathbf{z}} \gets \hat{\mathbf{z}}_{\phi}(\mathbf{z}_t,\mathbf{z}_l,\lambda_t)$ \Comment{Obtain the target from teacher}
    \State $\mathcal{L}_\theta \gets \omega(\lambda_t)\|\hat{\mathbf{z}}_{\theta}(\mathbf{z}_t,\mathbf{z}_l,\lambda_t) - \tilde{\mathbf{z}}\|_2^2$
    \State $\theta \gets \theta - \eta \nabla_\theta \mathcal{L}_\theta$
\EndWhile

\end{algorithmic}
\caption{Architecture Distillation Training. $\Call{Degrade}$ function degrades a given HR image with the given scale factor. $\Call{ResizeLike}$ function resizes a given LR image to the same size as the given HR image using the bicubic method.}
\label{alg:ad}
\end{algorithm}

\paragraph{Smaller UNet model.} We begin by describing the proposed small SD-SR architecture adapted here. We start from the UNet model of SD 1.5\footnote{https://huggingface.co/runwayml/stable-diffusion-v1-5}, which we rely on in the main paper, and consider various approaches to yield a smaller architecture. In particular, we considered three main approaches to reduce the model size: \textbf{i)} skipping residual blocks, \textbf{ii)} removing attention layers and \textbf{iii)} reducing the number of channels in each layer. Our initial explorations revealed that reducing the number of channels resulted in the highest gain in terms of parameters. Therefore, our final small model was obtained by removing $50\%$ of the channels, thereby reducing the number of parameters from $860$M parameters to $158$M. Unfortunately, training $158$M model for $\times 4$ magnification results in a severe drop in performance compared to the big $860$M model; see the first row of Tab.~\ref{tab:arch-distill}. Like the big model, training the same small model with scale distillation on the small model improves the performance remarkably; see the second row in Tab.~\ref{tab:arch-distill}. To close the gap with the best $860$M model, we propose to perform architecture distillation and combine it with scale distillation in the following.



\paragraph{Architecture distillation.} A straightforward approach to improve the performance of the smaller model given a trained large model is to use the large model as a teacher to obtain the training target for the small student model. That is, to train the student at time step $t$, we feed the frozen big teacher with the same noisy and LR input image and use its prediction as a target to train the small student model. We call this procedure architecture distillation. As we show in the third row of Tab.~\ref{tab:arch-distill}, architecture distillation results in a better model compared to using the raw data as a target, compare the third row with the first row in Tab.~\ref{tab:arch-distill}. In the following, we show that combining the scale and architecture distillation further improves the performance. Alg.~\ref{alg:ad} explains the procedure in detail.

\paragraph{More effective scale distillation for the small model.} Due to the large gap between the large and small model capacities, the student model could potentially underfit during architecture distillation for a large scale factor, \eg $\times 4$ used in Tab.~\ref{tab:arch-distill}. To provide a more simplified supervisory signal for the student, we propose to perform architecture distillation on the lower scale factor, \eg $\times 2$, and use the resulting model as a teacher for scale distillation to train the final model for $\times 4$ magnification. The rationale behind our proposed approach is that when training a model for $\times 2$ magnification, the student has a simpler task. Therefore, it can mimic the big model teacher's behavior during the training more effectively. As a result, the gap between the small and big models for the $\times 2$ magnification is smaller compared to $\times 4$ magnification. We then use this model as a teacher for scale distillation for $\times 4$ magnification, \ie $\times 2 \rightarrow \times 4$. In summary, since architecture distillation archives better performance compared to training with raw data, we obtain a better $\times 2$ model via architecture distillation. Consequently, scale distillation from this teacher results in a better student for $\times 4$  compared to the case where the $\times 2$ model is trained on raw data for the initial scale, see the fourth row of Tab.~\ref{tab:arch-distill}.
